Solving the Job Shop Scheduling Problem with Graph Neural Networks: A Customizable Reinforcement Learning Environment

The job shop scheduling problem is an NP-hard combinatorial optimization problem relevant to manufacturing and timetabling. Traditional approaches use priority dispatching rules based on simple heuristics. Recent work has attempted to replace these with deep learning models, particularly graph neural networks (GNNs), that learn to assign priorities from data. However, training such models requires customizing numerous factors: graph representation, node features, action space, and reward functions. The lack of modular libraries for experimentation makes this research time-consuming. This work introduces JobShopLib, a modular library that allows customizing these factors and creating new components with its reinforcement learning environment. We trained several dispatchers through imitation learning to demonstrate the environment's utility. One model outperformed various graph-based dispatchers using only individual operation features, highlighting the importance of feature customization. Our GNN model achieved near state-of-the-art results on large-scale problems. These results suggest significant room for improvement in developing such models. JobShopLib provides the necessary tools for future experimentation.

==> chapters/Abstract.tex <==
The job shop scheduling problem is an NP-hard combinatorial optimization problem relevant to manufacturing and timetable scheduling. Because of the problem's combinatorial nature, heuristics are typically used. They aim to provide “good enough" solutions. One of the most common approaches is to use priority dispatching rules. These rules decide which tasks should be prioritized based on simple heuristics, such as choosing the one that finishes the earliest.

In recent years, there have been attempts to replace these rules with deep learning models, which learn to assign priorities through data. Specifically, graph neural networks have emerged as an alternative. However, numerous factors can be customized when generating training data: the graph used to represent the problem, the features used to represent each node, the definition of tasks available for dispatching at each moment, and the reward function used. Due to the lack of modular libraries that allow choosing and experimenting with new components, training such models requires significant investments in development time.

This work introduces a new modular library, JobShopLib, that incorporates a reinforcement learning environment that allows customizing each of these factors and creating new ones. Furthermore, several task selection models have been trained through imitation learning using this library's environment to show its utility. One of these models outperformed various graph-based dispatchers while considering only individual task features. This suggests that aspects such as node features are important, further justifying the need for customization that our library provides. Moreover, our graph neural network-based model has achieved very close to state-of-the-art results in large-scale problems. Both results suggest that there is still significant room for improvement in developing these types of models. \textit{JobShopLib}, with its environments for generating training data, aims to provide the tools for such future experimentation.


==> chapters/Acknowledgement.tex <==
A todos los profesores que se han preocupado tanto en que tuviéramos la mejor educación posible, llegando a trabajar y preparar clases que incluso iban más allá del temario estrictamente necesario. Creo que, por desgracia, la increíble calidad de educación que he recibido en esta escuela es algo muy inusual y estoy tremendamente agradecido por ello. Aunque me estoy dejando muchos nombres, me gustaría hacer una especial mención a Paco Gómez, a Jesús Bobadilla, a Carlos Quesada (de nuevo), a Alberto Díaz, y a Carlos Badenes por esta dedicación extraordinaria en las clases.

Al grupo de investigación Knodis y a mi tutor, Carlos, por ceder parte de sus recursos para que pueda realizar entrenamientos en sus servidores.

A mis amigos. En este aspecto se me hace imposible pensar que podría estar todavía mejor acompañado. Gracias por ayudarme a ver las cosas más claras, por apoyarme en los momentos más difíciles y por todas las risas y los buenos momentos que hemos vivido. Sin duda tengo que hacer una especial mención a Álvaro, mi compañero en casi todos los proyectos que hemos hecho en estos 4 años. Gracias por aguantarme y hacer esta carrera un poco más fácil. No quiero mencionar más nombres porque sois muchos los que me habéis apoyado y me sería injusto dejar fuera a nadie. Vosotros sabéis quienes sois. Os quiero :)

A mis padres. Por preocuparos tanto por mí y por todo el amor y apoyo que me dais todos los días.

Por último, a mi tutor (otra vez), Carlos. Este ha sido un proyecto ambicioso y sin tu confianza y apoyo no hubiera sido posible. Gracias también por todas las enseñanzas, por haber tenido tanta disponibilidad e interés, no solo en que este proyecto saliera adelante, sino también en que pudiera tener el mejor futuro posible una vez termine esta carrera.


==> chapters/Conclusions.tex <==
% Write your conclusions here
\label{Conclusions} % If you need a label for this chapter

\doublespacing % Do not change - required

This chapter reflects on the contributions and findings of this research project, assesses its limitations, and outlines promising directions for future work. 

\section{Project Successes and Contributions}
The primary objective of this thesis was to develop a flexible and extensible framework for exploring GNN-based approaches to the \ac{JSSP}, an aim that has been achieved through the creation of \textit{JobShopLib}---a versatile Python library—and two highly flexible Reinforcement Learning (RL) environments built upon it. These tools address a significant gap in \ac{JSSP} research: the lack of standardized, customizable frameworks for experimenting with different design choices in GNN-based dispatching.

\subsection{Development of \textit{JobShopLib}}
Supporting a modular and extensible \ac{RL} environment also requires a library to support these options. The development of \textit{JobShopLib} provides these environments with classes and modules that implement all the functionality needed. Moreover, by open-sourcing the individual components of this library, we also support ot of related applications that could benefit from other \textit{JobShopLib}'s components. For example, the flexibility of the dispatching rule framework also facilitates research on the creation of new \ac{PDRs}. The user would only need to define their rule, and they will automatically have access to multiple ready operation filters and built-in rules that could be used for running experiments.

Several users already use these components, as proved by the GitHub stars and interactions through issues. \textit{JobShopLib}'s documentation page, containing examples and an API reference for all classes and functions, further aids this adoption. 

\subsection{Empirical Findings}
Beyond the library, the project proved its practical value by training a GNN-based dispatcher with data generated using \textit{JobShopLib}'s \ac{RL} environment. The GNN learned to copy the decisions of an optimal \ac{CP} solver on small problems, successfully applying these learned patterns to larger instances---especially in the case of the \ac{RGATv2} model.

An important discovery was how much carefully designed node features affected performance. A baseline model, utilizing only \textit{JobShopLib}'s built-in features without GNN message passing, outperformed several existing GNN-based approaches. This shows the strength of the library's feature collection mechanism and demonstrates that advanced graph learning methods need to be compared to straightforward, feature-only-based alternatives.

\section{Limitations and Future Research Directions}
While this project achieved its primary objectives, it is important to acknowledge its limitations. These limitations present opportunities for future improvements and extensions to the library and the underlying methodologies.

\subsection{Ablation Studies}
While \textit{JobShopLib} supports a wide range of design choices, our experimental evaluation did not exhaustively explore all possible combinations. A comprehensive ablation study examining the interactions between different components (graph representations, node features, action space definitions, etc.) remains to be conducted.

A thorough investigation of the impact of different design choices would advance our understanding of GNN-based dispatching for \ac{JSSP}. \textit{JobShopLib} provides tools that facilitate:
\begin{itemize}[itemsep=0pt, topsep=0pt]
    \item Systematically comparing different graph representations (disjunctive graphs, Resource-Task graphs, and their variants) to determine which structures most effectively capture the problem's constraints and relationships.
    \item Evaluating the relative importance of node features and their interactions, potentially introducing more informative feature subsets.
    \item Further investigating the impact of various action space definitions.
    \item Comparing different reward functions for RL training.
\end{itemize}

\subsection{Extensions to Real-World Problems}
The current implementation has been tested on classical \ac{JSSP} instances with deterministic processing times. Extensions to dynamic or stochastic variants of the problem would require additional development and validation. \textit{JobShopLib} can still be further extended (especially its core data structures) to support more realistic scheduling environments.

Nevertheless, as discussed in \href{https://github.com/Pabloo22/job_shop_lib/issues/16}{this Github issue}, it is important to note that due to its modular design, many problem variants can be easily integrated. For example, support for due dates would only require adding that attribute to the \texttt{Operation} class (or a subclass). Then we can create a new \texttt{RewardObserver} that takes into account if there is any delay, and a new \texttt{FeatureObserver} to add this time as a node feature.


\subsection{Better GNN Architectures}
The performance differences shown between the \ac{RGATv2} model and \ac{RGIN}, combined with the strong performance of the Non-\ac{MP} baseline, suggest that design choices aimed to increase generalization need to be taken seriously. This hypothesis aligns with previous work in neural algorithmic reasoning. \cite{dudzik2022gnns_are_dps} argue that aligning GNN architectures with classical algorithms for solving the same problem can bring significant generalization improvements. Future work could explore architectures that better match the computation in classical solving methods, such as dynamic programming or \ac{CP}.

\section{Concluding Remarks}

This project has presented \textit{JobShopLib}, a comprehensive library for experimenting with GNN-based approaches to the \ac{JSSP}. By abstracting the key design choices identified in the literature, the library enables researchers to systematically explore the space of possible solutions and understand the factors that contribute to effective learning-based schedulers.

Our experiments have demonstrated that even relatively simple GNN models trained with imitation learning can achieve competitive performance on benchmark instances. Moreover, the expressive power of the built-in node features suggests that carefully designed representations can capture much of the relevant information for making effective scheduling decisions.

The modular architecture of \textit{JobShopLib} positions it as a valuable tool for advancing the state of the art in learning-based scheduling. By reducing the implementation burden associated with experimenting with different design choices, the library can accelerate progress toward more effective and practical scheduling systems.

As manufacturing and service industries continue to face increasing complexity and demands for flexibility, the flexibility of learning-based approaches to scheduling problems will become increasingly important. \textit{JobShopLib}, especially through its \ac{RL} environments, contributes to this goal by providing a foundation upon which researchers can build robust GNN schedulers.


==> chapters/ListAcronyms.tex <==
% Add your acronyms here

\begin{acronym}
 \acro{JSSP}{Job Shop Scheduling Problem}
 \acro{PDRs}{Priority Dispatching Rules}
 \acro{SPT}{Shortest Processing Time}
 \acro{MWKR}{Most Work Remaining}
 \acro{FCFS}{First Come First Served}
 \acro{MOR}{Most Operations Remaining}
 \acro{MILP}{Mixed Integer Linear Programming}
 \acro{CP}{Constraint Programming}
 \acro{ML}{Machine Learning}
 \acro{DL}{Deep Learning}
 \acro{NNs}{Neural Networks}
 \acro{tanh}{hyperbolic tangent}
 \acro{ReLU}{Rectified Linear Unit}
 \acro{ELU}{Exponential Linear Unit}
 \acro{SGD}{Stochastic Gradient Descent}
 \acro{ANNs}{Artificial Neural Networks}
 \acro{GNNs}{Graph Neural Networks}
 \acro{MP}{Message Passing}
 \acro{RGNNs}{Relational Graph Neural Networks}
 \acro{GCNs}{Graph Convolutional Networks}
 \acro{RGCNs}{Relational Graph Convolutional Networks}
 \acro{CNNs}{convolutional Neural Networks}
 \acro{GATs}{Graph Attention Networks}
 \acro{RGATv2}{Relational Graph Attention Network v2}
 \acro{GINs}{Graph Isomorphism Networks}
 \acro{RGIN}{Relational Graph Isomorphism Network}
 \acro{MLP}{Multilayer Perceptron}
 \acro{MDP}{Markov Decision Process}
 \acro{SMDP}{Semi-Markov Decision Process}
 \acro{RL}{Reinforcement Learning}
 \acro{IL}{Imitation Learning}
 \acro{BC}{Behavioral Cloning}
 \acro{A2C}{Advantage Actor-Critic}
 \acro{PPO}{Proximal Policy Optimization}
 \acro{PyG}{Pytorch Geometric}
 \acro{PE}{Periodic Embedding}
 % ADD MORE ACRONYMS AS NEEDED WITH
 % \acro{example}
 % WHEN YOU USE THE ACRONYM IN THE TEXT
 % USE THE COMMAND \ac{example}
\end{acronym}

==> chapters/Notation.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cl}
\hline
\textbf{Notation} & \textbf{Description} \\
\hline
$\mathcal{J}$ & Set of jobs \\
$\mathcal{M}$ & Set of machines \\
$|\mathcal{J}| \times |\mathcal{M}|$ & Problem size (number of jobs × number of machines) \\
$J_i$ & Job $i$ in set $\mathcal{J}$ \\
$O_{ij}$ & Operation $j$ of job $i$ \\
$M_j$ & Machine $j$ in set $\mathcal{M}$ \\
$p_{ij}$ & Processing time of operation $O_{ij}$ (also called duration) \\
$S_{ij}$ & Start time of operation $O_{ij}$ \\
$C_{ij}$ & Completion time of operation $O_{ij}$ ($C_{ij} = S_{ij} + p_{ij}$) \\
$C_{max}$ & Makespan (maximum completion time of all operations) \\
\hline
\end{tabular}
\caption{Job-Shop-Scheduling-Problem-related notation}
\label{tab:jssp_notation}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{cl}
\hline
\textbf{Notation} & \textbf{Description} \\
\hline
$G = (V, E, \mathbf{X})$ & Graph with nodes $V$, edges $E$, and feature matrix $\mathbf{X}$ \\
$\mathbf{x}_i$ & Feature vector of node $i$ \\
$\mathbf{h}_i$ & Hidden representation of node $i$ \\
$\mathcal{N}_i$ & Set of neighboring nodes of node $i$ \\
$\psi$ & Message function \\
$\phi$ & Update function \\
$\bigoplus$ & Permutation invariant aggregation operator \\
$\mathbf{W}^{(l)}$ & Learnable weight matrix at layer $l$ \\
$d_i$ & Degree of node $i$ \\
$\alpha_{ij}$ & Attention coefficient from node $j$ to node $i$ \\
$e_{ij}$ & Unnormalized attention score \\
$\mathbf{a}$ & Learnable attention vector \\
$K$ & Number of attention heads \\
$\epsilon^{(l)}$ & Learnable/fixed parameter in \ac{GINs} at layer $l$ \\
$\mathcal{R}$ & Set of relationship types in relational \ac{GNNs} \\
$\mathcal{N}^r_i$ & Set of neighbors of node $i$ connected through relationship type $r$ \\
$\mathbf{W}_r^{(l)}$ & Weight matrix specific to relationship type $r$ at layer $l$ \\
\hline
\end{tabular}
\caption{Graph-Neural-Network-related notation}
\label{tab:gnn_notation}
\end{table}

\begin{table}[htbp]
\centering
\begin{adjustwidth}{-1cm}{}
\begin{tabular}{cl}
\hline
\textbf{Notation} & \textbf{Description} \\
\hline
$\mathcal{S}$ & Set of states \\
$\mathcal{A}$ & Set of actions \\
$P$ & Transition probability function ($P(s'|s,a)$ is prob. of $s \xrightarrow{a} s'$) \\
$R$ & Reward function ($R(s,a,s')$ is reward for $s \xrightarrow{a} s'$) \\
$\gamma$ & Discount factor \\
$s, s_t, s_k$ & State (at a general, specific time step $t$, or decision $k$) \\
$a, a_t, a_k$ & Action (at a general, specific time step $t$, or decision $k$) \\
$s'$ & Next state (resulting from state $s$ and action $a$) \\
$\pi$ & Policy (mapping from states to actions or action probabilities) \\
$J(\pi)$ & Objective function; expected cumulative discounted reward for policy $\pi$ \\
$F$ & Sojourn time distribution in SMDP ($F(s, a, s', \tau)$ is prob. transition $s \xrightarrow{a} s'$ takes time $\tau$) \\
$\tau$ & Time duration of a state transition in an SMDP \\
$t_k$ & Time at which the $k$-th decision is made (in SMDP, for discounting variable duration steps) \\
$V^{\pi}(s)$ & State-value function: expected return from state $s$ following policy $\pi$ \\
$Q^{\pi}(s,a)$ & Action-value function: expected return from state $s$, taking action $a$, then following $\pi$ \\
$A^{\pi}(s,a)$ & Advantage function: $Q^{\pi}(s,a) - V^{\pi}(s)$ \\
$\theta$ & Learnable parameters of a function approximator (e.g., for a policy) \\
$\pi_{\theta}(a|s)$ & Policy parameterized by $\theta$; outputs probability of taking action $a$ in state $s$ \\
$\nabla_{\theta}J(\pi_{\theta})$ & Gradient of the objective $J$ with respect to policy parameters $\theta$ \\
$d^{\pi}$ & On-policy state distribution under policy $\pi$ \\
$G_t$ & Return: sum of discounted rewards from time step $t$ onwards \\
$N$ & Number of data points (e.g., episodes in REINFORCE, expert state-action pairs in BC) \\
$B$ & Batch size for gradient updates (e.g., in A2C, PPO) \\
$L^{CLIP}(\theta)$ & Clipped surrogate objective function in PPO \\
$r_t(\theta)$ & Probability ratio $\frac{\pi_\theta(a_t|s_t)}{\pi_{\theta_{old}}(a_t|s_t)}$ in PPO, comparing current policy to old policy $\pi_{\theta_{old}}$ \\
$\epsilon$ & Hyperparameter in PPO defining the clipping range $(1-\epsilon, 1+\epsilon)$ \\
$\mathcal{D}_E$ & Dataset of expert demonstrations, typically pairs of $(s_i, a^*_i)$ \\
$a^*, a^*_i$ & Action taken by an expert (in state $s_i$) \\
$\theta^*$ & Optimal parameters for $\pi_\theta$ learned by minimizing the Behavioral Cloning loss \\
$L(\pi_\theta(s), a^*)$ & Loss function in Behavioral Cloning, measures dissimilarity between $\pi_\theta(s)$ and $a^*$ \\
$\mathcal{A}(s_k)$ & Set of available (candidate) actions in state $s_k$ \\
$y_{ij}$ & True label (e.g., 1 if operation $O_{ij}$ is an expert action, 0 otherwise) for BC in JSSP \\
$\hat{y}_{ij}$ & Predicted probability by $\pi_\theta$ that operation $O_{ij}$ is an expert action (BC for JSSP) \\
\hline
\end{tabular}
\end{adjustwidth}
\caption{Reinforcement Learning and Imitation Learning notation}
\label{tab:rl_il_ch4_notation}
\end{table}

==> chapters/OrigSta_Copyright.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT MODIFY FROM HERE ...
\cleardoublepage\phantomsection
\addcontentsline{toc}{chapter}{Declaration of Originality}\mtcaddchapter 
\chapter*{Declaration of Originality}
\addtocounter{counter}{-1}
% ... TO HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% EDIT FROM HERE
% Example text



I hereby declare that the work presented in this thesis is my own unless otherwise stated. To the best of my knowledge the work is original and ideas developed in collaboration with others have been appropriately referenced.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT MODIFY FROM HERE ...
\cleardoublepage\phantomsection
\addcontentsline{toc}{chapter}{Copyright Declaration}\mtcaddchapter 
\chapter*{Copyright Declaration}
\addtocounter{counter}{-1}
% ... TO HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% EDIT FROM HERE
% Example text

The copyright of this thesis rests with the author and is made available under the \href{https://creativecommons.org/licenses/by/4.0/}{Creative Commons Attribution 4.0 International (CC-BY-4.0)} license. This project is based on \href{https://www.overleaf.com/latex/templates/meng-beng-msc-report-template-eee-imperial-college-london-v1-dot-2-1/qtkpngktpwpw}{Giordano Scarciotti's thesis template}, but some modifications have been made. These changes include colors, logo, removing blank pages, and adding a ``Resumen'' section to comply with the Polytechnic University of Madrid's regulation.

==> chapters/Resumen.tex <==
El problema de programación de tareas en talleres (\textit{job shop scheduling problem}) es un problema de optimización combinatoria NP-difícil con una gran relevancia en sectores como la manufactura o en la programación de horarios. Debido a la naturaleza combinatoria del problema, normalmente se recurre a heurísticas. Estas buscan otorgar soluciones “suficientemente buenas". Una de las más comunes son las reglas de asignación de prioridad (\textit{priority dispatching rules}). Dichas reglas deciden que tareas deben ser priorizadas en base a heurísticas sencillas como elegir aquella que termine en menor tiempo.

En los últimos años, ha habido intentos de reemplazar estas reglas con modelos de aprendizaje profundo, los cuales aprenden a asignar prioridades a través de datos. Específicamente, las redes neuronales de grafos han surgido como una alternativa. Sin embargo, existen numerosos factores que pueden ser personalizados al generar los datos de entrenamiento: el grafo utilizado para representar el problema, las características (\textit{features}) usadas para representar cada nodo, la definición de las tareas disponibles para despacho en cada momento y la función de recompensa utilizada. Debido a la falta de librerías modulares que permitan elegir y experimentar con nuevos componentes, entrenar dichos modelos requiere inversiones significativas en tiempo de desarrollo.

Este trabajo introduce una nueva librería modular, \textit{JobShopLib}, que incorpora un entorno de aprendizaje por refuerzo que permiten personalizar cada uno de dichos factores, así como crear nuevos. Además, para demostrar su utilidad, se han entrenado varios modelos de selección de tareas mediante aprendizaje por imitación haciendo uso del entorno de esta librería. Uno de estos modelos es capaz de superar a varios modelos basados en grafos considerando únicamente características individuales de cada tarea. Esto sugiere que aspectos como las características de los nodos son importantes, justificando aún más la necesidad de personalización que proporciona nuestra librería. Por otro lado, nuestro modelo basado en redes neuronales de grafos ha conseguido resultados muy cercanos al estado de la cuestión en problemas de tamaño grande. Ambos resultados sugieren que existe todavía un margen de mejora amplio en el desarrollo de este tipo de modelos. \textit{JobShopLib}, con sus entornos para la generación de datos de entrenamiento, pretende aportar las herramientas necesarias para dicha experimentación futura.
